Decoding Human-LLM Collaboration in Coding: An Empirical Study of Multi-Turn Conversations in the Wild

Large language models (LLMs) are increasingly acting as dynamic conversational interfaces, supporting multi-turn interactions that mimic human-like conversation and facilitate complex tasks like coding. While datasets such as LMSYS-Chat-1M and WildChat capture real-world user-LLM conversations, few studies systematically explore the mechanisms of human-LLM collaboration in coding scenarios. What tortuous paths do users experience during the interaction process? How well do the LLMs follow instructions? Are users satisfied? In this paper, we conduct an empirical analysis on human-LLM coding collaboration using LMSYS-Chat-1M and WildChat datasets to explore the human-LLM collaboration mechanism, LLMs' instruction following ability, and human satisfaction. This study yields interesting findings: 1) Task types shape interaction patterns(linear, star and tree), with code quality optimization favoring linear patterns, design-driven tasks leaning toward tree structures, and queries preferring star patterns; 2) Bug fixing and code refactoring pose greater challenges to LLMs' instruction following, with non-compliance rates notably higher than in information querying; 3) Code quality optimization and requirements-driven development tasks show lower user satisfaction, whereas structured knowledge queries and algorithm designs yield higher levels. These insights offer recommendations for improving LLM interfaces and user satisfaction in coding collaborations, while highlighting avenues for future research on adaptive dialogue systems. We believe this work broadens understanding of human-LLM synergies and supports more effective AI-assisted development.

==> copy/2_bg.tex <==
% \section{Related Work}
% \song{add a Section "LLM-based Coding"}

% \song{merge 2.1 and 2.2}
% \subsection{Multi-Turn Interaction Analysis}
% Prior research has explored multi-turn interactions between humans and LLMs in various contexts, particularly focusing on simulated environments and performance evaluations.
% ~\citet{mozannar2023simulating} employed LLMs, such as GPT-3.5, to simulate interactions between human programmers and AI assistants during programming tasks. In this simulated setting, they found that the coding capabilities of LLMs of varying scales correlate with their performance in these interactions.
% ~\citet{laban2025llms} decomposed complete single-turn instructions into fragmented pieces to construct a fragmented simulation environment. They conducted a systematic evaluation of mainstream LLMs across six generative tasks, including database querying, mathematical reasoning, and text generation, with a focus on performance degradation in scenarios with incomplete instructions. Their findings reveal that once LLMs veer off course in dialogues, they become disoriented and fail to recover.
% ~\citet{han2025c} examined LLMs' handling of multi-turn entangled or conflicting instructions using a human-constructed dialogue dataset with three difficulty levels (e.g., instruction retrieval, cross-turn inference) and nine capability tasks (e.g., memory, dynamic instructions). They found no model excels in all tasks and that attention mechanisms fail to integrate multi-turn instructions effectively, despite decent retention.
% ~\citet{deng2024multi} introduced Self-MAP for dialogue-based web navigation, integrating memory retrieval, reflective optimization, and multifaceted planning. Experiments demonstrated superior performance over baselines in element accuracy and turn success rates, emphasizing the importance of memory and self-reflection in complex tasks.


% Our work differs from these studies in several key ways. While existing efforts predominantly rely on simulated environments or controlled datasets to assess LLM performance in multi-turn interactions, we emphasize empirical analysis of real-world human-LLM collaborations in coding tasks, drawing from large-scale datasets like LMSYS-Chat-1M and WildChat. Rather than focusing solely on model capabilities or methodological enhancements, we dissect interaction patterns, task types, and user satisfaction dynamics to uncover practical insights into collaboration mechanisms, including the impacts of instruction compliance and evolving user experiences.



% \subsection{Multi-Turn Interaction Evaluation}
% \bin{Need to reduce}
% Multi-turn interaction data is also crucial for understanding real-world dynamics and evaluating LLMs in naturalistic settings.
% Researchers have assessed LLMs by gathering large-scale human-LLM interaction data from real-world scenarios.
% ~\citet{zheng2023lmsys} introduced the LMSYS-Chat-1M dataset, which aggregates one million authentic conversations from 210K unique IP addresses, involving 25 LLMs and spanning over 150 languages and diverse topics.
% ~\citet{zhao2024wildchat} presented the WildChat dataset, comprising over one million user-ChatGPT conversations across more than 2.5 million interaction turns, collected by offering free ChatGPT access with explicit user consent.
% Beyond collecting genuine user-LLM multi-turn data, some researchers leverage LLMs to simulate real users and generate multi-turn dialogue data for evaluation.
% ~\citet{kwan2024mt} developed MT-Eval by integrating real dialogue patterns into GPT-4-generated multi-turn conversations. Evaluations indicated performance degradation linked to greater information distance and error propagation, with most models faltering in memory and dynamic instruction tasks.
% ~\citet{bai2024mt} constructed MT-Bench-101, featuring a three-level capability hierarchy for fine-grained assessment of LLMs' multi-turn abilities. Results highlighted significant shortcomings in adaptability and interactivity.
% ~\citet{li2025structflowbench} introduced six dialogue relations—Follow-up, Refinement, Recall, Expansion, and others—to capture intrinsic conversational logic, building StructFlowBench to evaluate existing LLMs.
% ~\citet{kong2023platolm} proposed the SocraticChat dataset, fine-tuning a user simulator called Socratic on real human prompts, followed by iterative interactions between Socratic and ChatGPT to generate multi-turn dialogues.
% ~\citet{sun2024parrotenhancingmultiturninstruction} first trained the Parrot-Ask model on 70K ShareGPT conversations, then used it to interact with ChatGPT, yielding the Parrot-40K dataset with an average of 8.71 turns per conversation.
% ~\citet{fan2024fairmt} created the FairMT-10K fairness dataset to evaluate LLMs' fairness in multi-turn dialogues. Experiments demonstrated that LLMs are more prone to biased responses in multi-turn scenarios, with biases accumulating over turns.




% % Our study differs from prior benchmarks by surpassing dataset curation and simulated LLM evaluations, instead empirically analyzing real-world coding collaborations in authentic datasets. We emphasize interaction patterns, task-specific hurdles, and satisfaction trajectories, elucidating the roles of instruction adherence and pattern dynamics in shaping outcomes.






%% ================================================


\section{Related Work}
\song{add a Section "LLM-based Coding"}

\song{merge 2.1 and 2.2}

\lin{Interaction or Collaboration?}

\subsection{Multi-Turn Interaction Evaluation}

Prior work has delved into multi-turn interactions between humans and LLMs. 
% 例如：融入真实世界对话模式的MT-Eval,
For instance, 

For instance, ~\citet{kwan2024mt} introduced MT-Eval, which integrates real-world dialogue patterns into GPT-4 to generate multi-turn conversations. 
Similarly, ~\citet{bai2024mt} developed MT-Bench-101, employing a fine-grained hierarchy with three capability levels to assess LLM multi-turn performance in detail. 
~\citet{li2025structflowbench} introduced StructFlowBench, which defines six types of dialogue relations to model the underlying logic in conversations.
~\citet{fan2024fairmt} presented FairMT-10K to evaluate fairness in LLMs during multi-turn dialogues.
~\citet{sun2024parrotenhancingmultiturninstruction} trained a specialized Parrot-Ask model to simulate user-generated multi-turn exchanges for evaluating LLM behavior.
~\citet{mozannar2023simulating} simulated programmer-AI collaborations using GPT-3.5, revealing that LLM scale directly influences interaction effectiveness in coding tasks.
~\citet{han2025can} examined LLMs on entangled multi-turn instructions via a human-curated dataset spanning difficulty levels (e.g., retrieval, inference) and capabilities (e.g., memory); no model dominated, and attention mechanisms proved inadequate for cross-turn integration despite solid recall.
~\citet{laban2025llms} decomposed complete single-turn instructions into fragmented pieces to mimic incomplete scenarios, evaluating mainstream LLMs across tasks like database querying and math reasoning.Their findings reveal that once LLMs veer off course in dialogues, they become disoriented and fail to recover.


Beyond relying on LLMs to mimic real-user dialogue behaviors for assessing LLM performance, several efforts have turned to gathering interaction data from genuine conversational contexts.
For instance, ~\citet{zheng2023lmsys} collected the LMSYS-Chat-1M dataset, which compiles one million authentic conversations from over 210K unique IP addresses, engaging 25 LLMs across more than 150 languages and a wide range of topics. 
Similarly, ~\citet{zhao2024wildchat} compiled over one million user-ChatGPT dialogues, encompassing more than 2.5 million interaction rounds.

While existing efforts predominantly rely on simulated environments or controlled datasets to assess LLM performance in multi-turn interactions, we emphasize empirical analysis of real-world human-LLM collaborations in coding tasks, drawing from large-scale datasets like LMSYS-Chat-1M and WildChat. Rather than focusing solely on model capabilities or methodological enhancements, we dissect interaction patterns, task types, and user satisfaction dynamics to uncover practical insights into collaboration mechanisms, including the impacts of instruction compliance and evolving user experiences.

% ~\citet{zheng2023lmsys} introduced the LMSYS-Chat-1M dataset, which aggregates one million authentic conversations from 210K unique IP addresses, involving 25 LLMs and spanning over 150 languages and diverse topics.
% ~\citet{zhao2024wildchat} presented the WildChat dataset, comprising over one million user-ChatGPT conversations across more than 2.5 million interaction turns, collected by offering free ChatGPT access with explicit user consent.



\subsection{LLM-based Coding}




Multi-turn interaction data is also crucial for understanding real-world dynamics and evaluating LLMs in naturalistic settings.
Researchers have assessed LLMs by gathering large-scale human-LLM interaction data from real-world scenarios.





% Beyond collecting genuine user-LLM multi-turn data, some researchers leverage LLMs to simulate real users and generate multi-turn dialogue data for evaluation.

% constructed MT-Bench-101, featuring a three-level capability hierarchy for fine-grained assessment of LLMs' multi-turn abilities. Results highlighted significant shortcomings in adaptability and interactivity.
%  introduced six dialogue relations—Follow-up, Refinement, Recall, Expansion, and others—to capture intrinsic conversational logic, building StructFlowBench to evaluate existing LLMs.

% ~\citet{kong2023platolm} proposed the SocraticChat dataset, fine-tuning a user simulator called Socratic on real human prompts, followed by iterative interactions between Socratic and ChatGPT to generate multi-turn dialogues.
 % first trained the Parrot-Ask model on 70K ShareGPT conversations, then used it to interact with ChatGPT, yielding the Parrot-40K dataset with an average of 8.71 turns per conversation.
 % created the FairMT-10K fairness dataset to evaluate LLMs' fairness in multi-turn dialogues. Experiments demonstrated that LLMs are more prone to biased responses in multi-turn scenarios, with biases accumulating over turns.

% Our study differs from prior benchmarks by surpassing dataset curation and simulated LLM evaluations, instead empirically analyzing real-world coding collaborations in authentic datasets. We emphasize interaction patterns, task-specific hurdles, and satisfaction trajectories, elucidating the roles of instruction adherence and pattern dynamics in shaping outcomes.


% Prior research has explored multi-turn interactions between humans and LLMs in various contexts, particularly focusing on simulated environments and performance evaluations.


% ~\citet{deng2024multi} proposed Self-MAP for web navigation dialogues, incorporating memory retrieval and self-reflection, which outperformed baselines in accuracy metrics and underscored the value of these features in intricate exchanges.











==> copy/4_pattern.tex <==
\section{RQ1: Interaction Pattern}
\subsection{Methodology}
We first identified the task types and instruction intents in multi-turn conversation data using an open card sorting method. 
Specifically, we formed an expert analysis team and a student annotation team. 
Our expert analysis team includes four PhDs in Software Engineering or Computer Science, each with over 10 years of development experience (Java, Python) and extensive research expertise in intelligent software engineering and LLMs. The student annotation team comprises four graduate students in intelligent software engineering, whose 3+ years of development experience ensures that they can accurately interpret user and developer instructions for the annotation task.

%The expert analysis team consists of four experts with doctoral degrees in software engineering or computer science. 
%These experts possess extensive experience in intelligent software engineering and LLM-related research, along with over ten years of development expertise in Java and Python, providing them with deep insights into the domain. 
%The student annotation team comprises four graduate students from the field of intelligent software engineering, each with more than three years of software development experience. 
%This background enables them to effectively interpret instructions from typical users and developers, laying a solid foundation for the subsequent annotation tasks.


\textbf{Step 1: Exploratory analysis by the expert team.} 
The experts randomly selected 80 conversations from the multi-turn conversation samples (378) and conducted exploratory analysis using open card sorting. Each conversation serves as an independent "card." 
The four experts were divided into two random groups and thoroughly examined each conversation to determine its primary task type and the user's instruction intent. 
%Since we decouple the data, each conversation contains only one task type. 
%In cases where a conversation includes multiple task types, we retain only the dominant one to ensure consistency and comparability. 
\bin{Since the data was decoupled, each conversation was reduced to a single task type. For any remaining conversations with multiple task types, we retained only the dominant one to ensure consistency and comparability.} 
Our initial observations indicate that user instructions within conversations typically exhibit a single intent. 
During analysis, experts engaged in thorough discussions to resolve any disagreements until a consensus was reached. 
Ultimately, they identified 5 task types (encompassing 12 subtypes) and 11 instruction intents. 
%To verify the consistency of the analysis process, we compute Cohen's Kappa, yielding a value of 0.78.
\bin{The analysis process demonstrated substantial consistency, with a Cohen's Kappa of 0.78.}


\textbf{Step 2: Annotation by the student team.} 
Building on the task types derived from the exploratory analysis, the student annotation team independently annotates the remaining 298 samples. 
%The four students divide into two groups, with two graduate students per group. Each annotator assesses the card content based on their understanding and assigns the appropriate task type.
%We collect the annotation results from both student groups and perform initial statistical analysis. 
%For classification conflicts that arise during annotation, we retain the disputed cards and organize group discussions among team members, facilitating extensive exchanges and arguments until achieving agreement.
%If new task types emerge during annotation, the student team consults with the expert analysis team for in-depth discussion and confirmation of inclusion. 
%To further evaluate inter-annotator consistency, we calculate Cohen's Kappa for each team, resulting in an average value of 0.85, which demonstrates high reliability and stability in the annotation outcomes. 
%Through this systematic analysis, we obtain a total of 5 task types (encompassing 12 subtypes) and 11 instruction intents. As shown in Table xx.
\bin{ The four graduated students were equally divided into two groups. Annotators in each group individually assessed each card's content and assigned it a task type.
We then collected the results from both groups for initial statistical analysis. Disagreements in classification were resolved through moderated group discussions until a consensus was reached. 
If a potential new task type emerged, the student team consulted with the expert analysis team to confirm its validity and inclusion.
To ensure annotation quality, we evaluated inter-annotator reliability by calculating Cohen's Kappa for each group. The average Kappa was 0.85, indicating substantial agreement. This systematic process yielded a final set of 5 task types (with 12 subtypes) and 11 instruction intents, as detailed in Table xx.}

%Next
Subsequently, we modeled the human-LLM interaction process using graph theory to describe interaction patterns formally.

%% 交互模式的形式化定义  --- todo
\bin{formanlly pattern}

\textbf{Basic Graph Model Definition}
Let $G = (V, E)$ denote a directed acyclic graph that represents a complete interaction dialogue, where $V$ is the set of nodes, and each node $v\in V$ corresponds to an interaction turn, formalized as an ordered pair $v= (q_{u},r_{i})$.
Here, $q_{u}$ is the user's query text, and $r_{i}$ is the LLM's response text. Each node $v$ encapsulates the minimal unit of interaction, ensuring independence and traceability for every turn. 
The total number of nodes $\left | V \right |$ indicates the dialogue length.

The set $ E \subseteq V \times V $ comprises directed edges, where an edge $ (u, v) \in E  $ signifies that turn $v$ directly follows turn $u$, meaning the user query in $v$ semantically depends on the LLM response in $u$.

We introduce a virtual root node $v_0 \notin V$  (containing no actual interaction content) and add edges $(v_0, v_r) $ to all actual root nodes $v_r$ (nodes with in-degree 0), thereby extending the graph to \( G' = (V \cup \{v_0\}, E \cup \{(v_0, v_r) \mid \deg^-(v_r) = 0\}) \). This ensures a single root node. 
Termination nodes (with out-degree 0) represent the absence of further interaction.
Based on this graph model, we formalize three primary interaction patterns, each defined through the topological structure of the graph, which remains a directed acyclic graph.


\textbf{Linear Pattern}
The extended graph \( G' \) forms a directed path, featuring a unique sequence of nodes \( v_0, v_1, v_2, \dots, v_n \) (where \( n = |V| \geq 0 \)), such that \( E' = \{(v_i, v_{i+1}) \mid 0 \leq i < n\} \). In this structure, the root node \( v_0 \) has in-degree 0 and out-degree 1 (if \( n > 1 \)); the termination node \( v_n \) has in-degree 1 (if \( n > 1 \)) and out-degree 0; and all intermediate nodes \( v_i \) (for \( 0 < i < n \)) have in-degree and out-degree both equal to 1. The graph contains no cycles or branches, with a unique path of length \( n \) and diameter \( n \).


\textbf{Star Pattern}
The extended graph \( G' \) forms a directed star, featuring a unique central node \( v_0 \), such that \( E' = \{(v_0, v_i) \mid v_i \in V\} \). In this structure, the central node \( v_0 \) has in-degree 0 and out-degree \( |V| \); all leaf nodes \( v_i \) have in-degree 1 and out-degree 0. The graph contains no cycles or crossing edges, with depth 1 (all paths have length at most 1) and diameter 1.


\textbf{Tree Pattern}
The extended graph \( G' \) forms a directed tree, constituting a connected acyclic directed graph with a unique root node \( v_0 \) (in-degree 0), where the path from \( v_0 \) to any other node is unique. In this structure, the root node \( v_0 \) has in-degree 0 and out-degree at least 0; all non-root nodes have in-degree exactly 1 and out-degree at least 0 (permitting branches).



Finally, we employed the Kruskal-Wallis H test combined with Dunn's post-hoc test to analyze the relationships among task types, interaction turns, and interaction patterns. 
This approach suits data with long-tail and non-normal distributions, enabling non-parametric evaluation of inter-group differences.


% The Kruskal-Wallis H test serves as a non-parametric statistical method for comparing the medians of three or more independent sample groups to determine if significant differences exist. 
% It acts as a non-parametric alternative to one-way analysis of variance (ANOVA), proving particularly useful when data fail to meet assumptions of normality or homogeneity of variance. 
% Specifically, this test ranks all samples and computes the rank sum statistic H to assess inter-group differences. 
% The H value approximates a chi-square distribution, allowing computation of a p-value to decide whether to reject the null hypothesis (that all group medians are equal).


% Dunn's post-hoc test constitutes a multiple comparison procedure applied after the Kruskal-Wallis H test identifies significant inter-group differences. It facilitates pairwise comparisons to pinpoint which specific group pairs exhibit statistically significant differences. 
% This test relies on standardized rank differences and incorporates Bonferroni correction or other adjustments to control the false positive rate in multiple comparisons, thereby ensuring the accuracy and reliability of the results.

% \bin{Are these introductions able to be shorter?}

% 实验结果
\subsection{Result and analysis}

% 交互模式
\subsubsection{Interaction Patterns.}
This study identifies three primary human-LLM interaction patterns, as illustrated in Figure XX. Except for the root node, each node represents the i-th turn in the conversation and encompasses both the user prompt and the LLM response. Arrows denote dependencies between consecutive interaction turns.

\textbf{P1: Linear Pattern.}
Interactions proceed in a sequential, step-by-step manner, where each turn directly depends on the output of the preceding one. This pattern employs a linearly progressive structure to maintain coherence and logical flow in information transfer.

\textbf{P2: Star Pattern.}
Interactions revolve around a central theme or instruction, from which multiple related dialogue branches emerge. Each branch remains independent of the others while maintaining a connection to the central theme.

\textbf{P3: Tree Pattern.}
Interactions originate from an initial theme or instruction serving as the root node, gradually expanding into multiple branches and sub-branches to form a hierarchical structure. Each branch path constitutes an independent exploratory direction, yet the overall structure relies on outputs from upper-level nodes. This pattern leverages a tree-like progressive organization.


%% 插入交互模式图片
\bin{pattern fig}

%轮次与交互模式
\subsubsection{Turns and Patterns.}
%We examine the relationship between interaction turns and interaction patterns. First, we apply the Kruskal-Wallis H test, which yields a p-value of 3.3042e-27 (<0.05), indicating significant overall differences in the distribution of turns across different interaction patterns. This indicates that at least one pattern differs markedly from the others in terms of median turns. Subsequently, pairwise comparisons via Dunn's post-hoc test (with Bonferroni p-value correction) pinpoint the specific sources of these differences. As shown in Table XX, the p-value between the linear and tree patterns stands at 4.1771e-27 (<0.05), and that between the star and tree patterns at 3.5661e-15 (<0.05), while no significant difference emerges between the linear and star patterns. These results imply that the turn distributions for linear and star patterns exhibit high similarity, whereas the tree pattern distinctly diverges from both, typically associating with longer interaction turns.
\bin{We examined the relationship between interaction turns and interaction patterns using a Kruskal-Wallis H test. The test reveals a significant overall difference in the distribution of turns across patterns (p < 0.05), indicating that the median turn count of at least one pattern differed from the others.
To identify specific differences, we conducted Dunn's post-hoc test with Bonferroni correction. The results, shown in Table XX, indicates that the tree pattern had significantly more interaction turns than both the linear (p < 0.05) and star (p < 0.05) patterns. In contrast, no significant difference was found between the linear and star patterns.
These findings suggest that while linear and star patterns have similar turn counts, the tree pattern is associated with distinctly longer interactions.
I don't know whether it's necessary to provide the exact p-value}

Figure XX illustrates the density and median of turn distributions across different modes. The linear and star modes exhibit similar distribution shapes, both featuring lower medians and narrower ranges. In contrast, the tree mode displays a broader distribution that extends toward higher turns, indicating higher medians and greater variability. This visually corroborates the statistical findings, confirming that the tree pattern tends to involve more turns and thus reflects higher interaction complexity.

To further delineate the relationship between turns and patterns, we observe that systematic shifts in pattern proportions as interaction turns increase. 
As detailed in Table XX, when turns=2, the linear pattern accounts for 82.4\%, star for 17.6\%, and tree for 0\%. This indicates that low-turn interactions are almost entirely dominated by the linear pattern. At turns=3, linear remains at 67.9\%, but tree emerges (14.3\%). At turns=4, linear drops to 38.1\%, and tree rises to 35.7\%, marking a transitional phase. For turns$\geq$ 5, tree predominates, for example, 60.9\% at turns=5 and 83.3\% at turns=8. Meanwhile, star nearly vanishes for turns$\geq$5 (proportion close to 0\%).


Figure XX depicts the evolution of interaction pattern probabilities with increasing turns. For turns<4, linear dominates. 
Turns=4 serves as a transition where patterns balance. For turns $\geq$ 5, the tree pattern becomes prevalent (probability exceeding 60\%). 
This trend underscores that as interaction turns grow, human-LLM interaction complexity escalates, driving a shift from simple linear patterns toward more branched tree patterns.


%% 插入标准化残差表 + 对应图
\bin{Dunn xiaotiqin fig + tab}

% finding 1
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 1:}
Linear patterns dominate when the number of turns is $\leq$ 4 (with turns = 4 serving as a critical transition point for pattern shifts). Tree patterns prevail when the number of turns is $\geq$ 5.

\end{tcolorbox}






% 任务 与交互模式
\subsubsection{Tasks and Patterns}

We explored the associations between task types and interaction patterns based on the results of Fisher's exact test and standardized residuals analysis.
%First, Fisher's exact test produces a p-value of 0.0016 (<0.05), offering sufficient statistical evidence to reject the null hypothesis of independence between task types and interaction patterns. Instead, a significant association emerges, implying that different task types in human-LLM interactions favor particular patterns, which in turn shape the structure and complexity of these interactions. Next, we pinpoint specific association patterns via the standardized residuals table. Residuals with absolute values exceeding 1.96 denote significant deviations, whereas those above 1.0 in absolute value highlight noteworthy tendencies. As detailed in Table XX. For code quality optimization tasks, the residual with the star pattern stands at -2.681 (absolute value > 1.96), indicating a significant avoidance of the star pattern, while showing a lean toward the linear pattern (residual 1.392 > 1.0). This indicates that code quality optimization—such as code fixing or refactoring—generally demands systematic, incremental analysis and iterative refinements. The linear pattern accommodates ongoing contextual dependencies, steering clear of the star pattern's divergent, multi-directional explorations.
\bin{A Fisher's exact test reveals a significant association between task types and interaction patterns (p = 0.0016). We analyzed standardized residuals to pinpoint specific relationships (see Table XX), where absolute values >1.96 indicate significance and >1.0 suggest a tendency. For instance, "code quality optimization" significantly avoids the star pattern (residual = -2.68) while favoring the linear pattern (residual = 1.39), as its systematic, incremental nature suits contextual tasks like code refactoring over the star pattern's divergent explorations.I shortened a lot, you can check whether I lost any key information}

%Second, query information tasks yield a residual of 2.520 with the star pattern (absolute value > 1.96), revealing a significant preference for the star pattern. These tasks frequently entail retrieving information or addressing queries from diverse perspectives, where the star pattern supports divergent interactions centered on a core theme, such as branching from one knowledge point to interconnected ones. This underscores users' propensity for exploratory exchanges in knowledge-dense contexts.
\bin{Similarly, "query information" tasks showed a strong preference for the star pattern (residual = 2.520), as its divergent structure is ideal for exploratory exchanges, such as branching from a core topic to retrieve information from multiple perspectives.} 

%Moreover, while falling short of the significance threshold, other tasks exhibit discernible tendencies. Design-driven development tasks present a residual of 1.561 with the tree pattern (> 1.0) and -1.222 with the star pattern (absolute value > 1.0), signaling a preference for the tree pattern alongside avoidance of the star pattern. This points to users in design-driven development tasks favoring the tree pattern's multi-branched framework to enable iterative exploration and problem breakdown. In this context, the tree pattern originates from a central design challenge and progressively unfolds into multiple sub-paths, adeptly managing the inherent intricacies of system-level development. Environment configuration tasks display a residual of 1.504 with the star pattern (> 1.0), suggesting a inclination toward the star pattern. This likely arises because configuration challenges necessitate divergent trials around a focal issue. The star pattern enables swift multi-directional experiments without necessitating profound branching. Finally, requirement-driven development tasks feature small absolute residuals (all < 1.0), exhibiting neither significant nor notable tendencies, which indicates greater flexibility in their interaction patterns.
\bin{Other tasks showed notable, though not significant, tendencies (|residual| > 1.0). Design-driven development favored the tree pattern (residual = 1.561) while avoiding the star pattern (residual = -1.222), as the tree’s branching structure is well-suited for iterative problem breakdown in complex design. In contrast, environment configuration tasks leaned toward the star pattern (residual = 1.504), likely because its divergent trials are effective for troubleshooting a central issue. Finally, requirement-driven development showed no clear pattern preference (all |residuals| < 1.0), suggesting greater interaction flexibility.}



%% 插入标准化残差表 + 对应图
\bin{biaozhun fig + tab}

% finding 1
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 2:}
Our findings reveal that task types significantly influence the choice of interaction patterns. 
Specifically, code quality optimization tasks tend to avoid the star pattern and may depend more heavily on the Linear pattern. 
In contrast, system-level development tasks favor the tree pattern. Meanwhile, knowledge query tasks and environment configuration tasks lean towards the star pattern.

\end{tcolorbox}



\subsubsection{Turns and Task Impact on Patterns}

We further investigate the influence of interaction turns and task types on interaction patterns. Table XX stratifies the percentage distributions of interaction patterns %(linear, star, tree) 
by task type and turn length (Low: $\leq$ 4 turns; High: > 4 turns). Under low turns %( $\leq$ 4 )
\bin{deleted some brackets('()')}, all task types predominantly feature the linear pattern, with proportions ranging from 52.9\% (environment configuration) to 86.8\% (code quality optimization). For code quality optimization tasks, the linear pattern accounts for 86.8\%, star for 5.9\%, and tree for 7.4\%. This arises because the initial stages of code optimization often focus on localized fixes, allowing efficient iterative validation without introducing branching paths. Similarly, requirement-driven development exhibits a linear proportion of 74.7\%. This likely stems from straightforward user requirements, such as generating short code snippets, which a linear progression adequately addresses. In contrast, the star pattern appears more prominent in information query (28.7\%) and environment configuration (35.3\%) tasks, indicating a tendency for divergent exploration in short interactions, such as multi-dimensional knowledge queries. The tree pattern generally accounts for less than 13\% across task types, a finding that underscores the preference for simpler structures in constrained conversations. This low prevalence further illustrates that in short interactions %comprising fewer than 4 turns
, users gravitate toward direct, linear progression as a means to swiftly accomplish their objectives. 


The distribution shifts markedly under high turns %(turns>4)
, with the tree pattern dominating all tasks at proportions from 50.0\% (code quality optimization) to 75.0\% (environment configuration). In design-driven development, the tree pattern accounts for 64.7\%, while the linear pattern drops to 29.4\%. %This reflects the inherent nature of design-driven development tasks, which typically begin with overall architecture or functionality design, followed by modular implementation through branching paths.
\bin{This reflects the nature of design-driven development, which often starts with high-level design and proceeds to modular implementation via branching paths.}
In code quality optimization, the tree pattern reaches 50.0\%, primarily because it supports the construction of deep debugging chains. By comparison, information query tasks see the tree pattern surge to 61.5\%. %Notably, as turns increase, patterns evolve from star-like divergent structures in low turns to integrated tree structures. This suggests that persistent conversations in information queries often require nested sub-questions to build a comprehensive understanding. The star pattern nearly vanishes (mostly 0\%), while linear proportions decline to 25.0\%-50.0\%, reflecting how shallow explorations gradually transform into tree or linear forms in high turns, particularly in information query tasks.
\bin{Notably, as turns increase, interaction patterns evolve from star-like divergent structures to integrated tree structures. This suggests that persistent information query dialogues often require nested sub-questions to build a comprehensive understanding.
Correspondingly, the star pattern nearly disappears (mostly 0\%), while the linear pattern, though declining to 25.0\%–50.0\%, still maintains a notable presence. This indicates that even in deep information-seeking conversations, some shallow explorations continue in a linear manner, particularly in information query tasks.}

As illustrated in Figure XX, these shifts appear in the density distributions of turns in patterns and task types. Linear modes concentrate at lower turns for most tasks. In contrast, tree modes extend toward higher turns. They exhibit broader variability in tasks such as design-driven development and environment configuration.



%% 插入标准化残差表 + 对应图
\bin{rain fig + tab}

% finding 1
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 3:}
Our findings demonstrate that interaction turns and task types collectively drive the evolution of interaction patterns.
In low-turn interactions (turns$\leq$ 4 ), all tasks predominantly adopt the linear pattern, with code quality optimization showing the highest proportion (86.8\%). The star pattern stands out in environment configuration (35.3\%) and information query (28.7\%) tasks.
In high-turn interactions (turns>4), all tasks shift to the tree pattern as the dominant form, with environment configuration reaching the peak (75.0\%); the linear pattern decreases to 25.0\%-50.0\%.

\end{tcolorbox}







==> copy/4_pattern_1.tex <==
\section{RQ1: Interaction Pattern}
\subsection{Methodology}
We first identified the task types and instruction intents in multi-turn conversation data using an open card sorting method \cite{}. 
Specifically, we formed an expert analysis team and a student annotation team. 
Our expert analysis team includes four PhDs in Software Engineering or Computer Science, each with over 10 years of development experience (Java, Python) and extensive research expertise in intelligent software engineering and LLMs. The student annotation team comprises four graduate students in intelligent software engineering, whose 3+ years of development experience ensures that they can accurately interpret user and developer instructions for the annotation task.


\textbf{Step 1: Exploratory analysis by the expert team.} 
The experts randomly selected 80 conversations from the multi-turn conversation samples (378) and conducted exploratory analysis using open card sorting. Each conversation serves as an independent "card." 
The four experts were divided into two random groups and thoroughly examined each conversation to determine its primary task type, the user's instruction intent, and the interaction pattern. 
Since the data was decoupled, each conversation was reduced to a single task type. For any remaining conversations with multiple task types, we retained only the dominant one to ensure consistency and comparability.
Our initial observations indicate that user instructions within conversations typically exhibit a single intent. 
Additionally, we also required drawing the topological structure of each dialogue.
During analysis, experts engaged in thorough discussions to resolve any disagreements until a consensus was reached. 
Ultimately, they identified 5 task types (including 12 subtypes), 11 instruction intents, and 3 primary interaction patterns.
The analysis process demonstrated substantial consistency, with a Cohen's Kappa of 0.78.


\textbf{Step 2: Annotation by the student team.} 
Building on the task types derived from the exploratory analysis, the student annotation team independently annotates the remaining 298 samples. 
The four graduated students were equally divided into two groups. Annotators in each group individually assessed each card's content and assigned it a task type.
We then collected the results from both groups for initial statistical analysis. Disagreements in classification were resolved through moderated group discussions until a consensus was reached. 
If a potential new task type emerged, the student team consulted with the expert analysis team to confirm its validity and inclusion.
To ensure annotation quality, we evaluated inter-annotator reliability by calculating Cohen's Kappa for each group. The average Kappa was 0.85, indicating substantial agreement. This systematic process yielded a final set of 5 task types (with 12 subtypes), 11 instruction intents, and 3 primary interaction patterns, as detailed in Table xx.

Subsequently, we employed the Kruskal-Wallis H test combined with Dunn's post-hoc test to analyze the relationships among task types, interaction turns, and interaction patterns. 
This approach suits data with long-tail and non-normal distributions, enabling non-parametric evaluation of inter-group differences.
\bin{add interactive pattern}

% 任务类型
\input{tab/task_type}

% 指令意图 -- 还没放
\input{}

% 实验结果
\subsection{Result and analysis}

\song{How do you identify the patterns? The above manual process focuses on labelling tasks, but does not mention the interaction patterns.}
% 交互模式
\subsubsection{Interaction Patterns.}
We have identified three primary interaction patterns, as illustrated in Figure  ~\ref{rq1_pattern}. 
Excluding the root, each node represents a conversational turn (including both user prompt and LLM response). Arrows denote dependencies between successive turns.
\textbf{(1) P1: Linear Pattern} advances sequentially, with each round building directly on the output of the previous round to ensure coherent information and logical flow.
\textbf{(2) P2: Star Pattern} centers on a core theme or root node, from which multiple independent branches derive, each maintaining a direct association with the center.
\textbf{(3) P3: Tree Pattern} originates from an initial theme or root node and progressively expands into multiple branches and sub-branches, forming a hierarchical structure; each branch path constitutes an independent exploration direction, with the overall structure relying on outputs from upper-level nodes.

\song{also need to show some statistical distributions of the patterns}

%% 交互模式图片
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq1_pattern.pdf}
    \caption{Interaction Patterns\song{explanations for ANF, FB, Q1...}} 
    \label{rq1_pattern}
    \vspace{-0.3cm}
\end{figure}




\song{4.2.2, 4.2.3, 4.2.4 all need a short motivation/connection to let readers know why you explore that point}


% 任务 与交互模式
\subsubsection{Tasks and Patterns}

We explored the associations between task types and interaction patterns based on the results of Fisher's exact test and standardized residuals analysis.
First, Fisher's exact test produces a p-value of 0.0016 (<0.05), offering sufficient statistical evidence to reject the null hypothesis.
We then analyzed the standardized residuals to determine specific relationships (see Table ~\ref{rq_1_std}), where absolute values greater than 1.96 indicate significance and greater than 1.0 indicates a tendency.
Specifically, code quality optimization significantly avoids the star pattern (residual = -2.68) while favoring the linear pattern (residual = 1.39), as its systematic, incremental nature suits contextual tasks like code refactoring over the star pattern's divergent explorations. 
Similarly, query information tasks showed a strong preference for the star pattern (residual = 2.520), as its divergent structure is ideal for exploratory exchanges, such as branching from a core topic to retrieve information from multiple perspectives.
Other tasks showed notable, though not significant, tendencies (|residual| > 1.0). 
Design-driven development favored the tree pattern (residual = 1.561) while avoiding the star pattern (residual = -1.222), as the tree’s branching structure is well-suited for iterative problem breakdown in complex design. 
In contrast, environment configuration tasks leaned toward the star pattern (residual = 1.504), likely because its divergent trials are effective for troubleshooting a central issue. 
Finally, requirement-driven development showed no clear pattern preference (all |residuals| < 1.0), suggesting greater interaction flexibility.

%% 插入标准化残差表
\input{tab/rq_1_std}


% finding 2
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 2:}
Task types significantly influence the choice of interaction patterns. 
Specifically, code quality optimization tasks tend to avoid the star pattern and may depend more heavily on the Linear pattern. 
In contrast, system-level development tasks favor the tree pattern. Meanwhile, knowledge query tasks and environment configuration tasks lean towards the star pattern.

\end{tcolorbox}



\subsubsection{Turns and Task Impact on Patterns}

We further investigate the influence of interaction turns and task types on interaction patterns. 
Table ~\ref{rq_1_fenceng} stratifies the percentage distributions of interaction patterns by task type and turn length (Low: $\leq$ 4 turns; High: > 4 turns). Under low turns, all task types predominantly feature the linear pattern, with proportions ranging from 52.9\% (environment configuration) to 86.8\% (code quality optimization). 
For code quality optimization tasks, the linear pattern accounts for 86.8\%, star for 5.9\%, and tree for 7.4\%. 
This arises because the initial stages of code optimization often focus on localized fixes, allowing efficient iterative validation without introducing branching paths. 
Similarly, requirement-driven development exhibits a linear proportion of 74.7\%. This likely stems from straightforward user requirements, such as generating short code snippets, which a linear progression adequately addresses. 
In contrast, the star pattern appears more prominent in information query (28.7\%) and environment configuration (35.3\%) tasks, indicating a tendency for divergent exploration in short interactions, such as multi-dimensional knowledge queries. 
The tree pattern generally accounts for less than 13\% across task types, a finding that underscores the preference for simpler structures in constrained conversations. 
This low prevalence further illustrates that in short interactions, users gravitate toward direct, linear progression as a means to swiftly accomplish their objectives. 


The distribution shifts markedly under high turns, with the tree pattern dominating all tasks at proportions from 50.0\% (code quality optimization) to 75.0\% (environment configuration). In design-driven development, the tree pattern accounts for 64.7\%, while the linear pattern drops to 29.4\%.
This reflects the nature of design-driven development, which often starts with high-level design and proceeds to modular implementation via branching paths.
In code quality optimization, the tree pattern reaches 50.0\%, primarily because it supports the construction of deep debugging chains. By comparison, information query tasks see the tree pattern surge to 61.5\%. 
Notably, as turns increase, patterns evolve from star-like divergent structures to integrated tree structures. This suggests that persistent information query dialogues often require nested sub-questions to build a comprehensive understanding.
Correspondingly, the star pattern nearly disappears (mostly 0\%), while the linear pattern, though declining to 25.0\%–50.0\%, still maintains a notable presence. This indicates that even in deep information-seeking conversations, some shallow explorations continue in a linear manner, particularly in information query tasks.


%%  分层的表
\input{tab/rq_1_fenceng}


% finding 3
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 3:}
Interaction turns and task types collectively drive the evolution of interaction patterns.
In low-turn interactions (turns$\leq$ 4 ), all tasks predominantly adopt the linear pattern, with code quality optimization showing the highest proportion (86.8\%). The star pattern stands out in environment configuration (35.3\%) and information query (28.7\%) tasks.
In high-turn interactions (turns>4), all tasks shift to the tree pattern as the dominant form, with environment configuration reaching the peak (75.0\%); the linear pattern decreases to 25.0\%-50.0\%.

\end{tcolorbox}

% 交互轮次与指令类型

\subsubsection{Turns and Patterns.}

We examined the relationship between interaction turns and interaction patterns. First, the Kruskal-Wallis H test yielded a p-value of 3.3042e-27 (<0.05), indicating a significant overall difference in the distribution of turns across different patterns. 
This indicates that the median turn count of at least one pattern differed significantly from the others.
Subsequently, pairwise comparisons were conducted using Dunn's post-hoc test (with Bonferroni correction). 
The results reveal significant differences in the round distributions between the tree pattern and both the linear (p=4.1771e-27) and star (p=3.5661e-15) patterns, whereas no significant difference exists between the linear and star patterns (p=1.0). 
This indicates that the linear and star patterns exhibit similar numbers of rounds, while the tree pattern typically involves longer interaction rounds.

To further delineate the relationship between turns and patterns, we observe that systematic shifts in pattern proportions as interaction turns increase. 
Figure ~\ref{turn-4} depicts the evolution of interaction pattern probabilities with increasing turns. For turns<4, linear dominates. 
Turns=4 serves as a transition where patterns balance. For turns $\geq$ 5, the tree pattern becomes prevalent (probability exceeding 60\%). 
This trend underscores that as interaction turns grow, human-LLM interaction complexity escalates, driving a shift from simple linear patterns toward more branched tree patterns.

%% turn-4
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/turn-4.pdf}
    \caption{Interaction Mode Probability Evolution by Turn} 
    \label{turn-4}
    \vspace{-0.4cm}
\end{figure}


% finding 1
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 1:}
Linear patterns dominate when the number of turns is $\leq$ 4 (with turns = 4 serving as a critical transition point for pattern shifts). Tree patterns prevail when the number of turns is $\geq$ 5.

\end{tcolorbox}








==> copy/4_pattern_meiyong.tex <==


% %  =============不用的==========


% This study identifies three primary human-LLM interaction patterns, as illustrated in Figure ~\ref{rq1_pattern}. Except for the root node, each node represents the i-th turn in the conversation and encompasses both the user prompt and the LLM response. Arrows denote dependencies between consecutive interaction turns.




%First, Fisher's exact test produces a p-value of 0.0016 (<0.05), offering sufficient statistical evidence to reject the null hypothesis of independence between task types and interaction patterns. Instead, a significant association emerges, implying that different task types in human-LLM interactions favor particular patterns, which in turn shape the structure and complexity of these interactions. Next, we pinpoint specific association patterns via the standardized residuals table. Residuals with absolute values exceeding 1.96 denote significant deviations, whereas those above 1.0 in absolute value highlight noteworthy tendencies. As detailed in Table XX. For code quality optimization tasks, the residual with the star pattern stands at -2.681 (absolute value > 1.96), indicating a significant avoidance of the star pattern, while showing a lean toward the linear pattern (residual 1.392 > 1.0). This indicates that code quality optimization—such as code fixing or refactoring—generally demands systematic, incremental analysis and iterative refinements. The linear pattern accommodates ongoing contextual dependencies, steering clear of the star pattern's divergent, multi-directional explorations.


%We examine the relationship between interaction turns and interaction patterns. First, we apply the Kruskal-Wallis H test, which yields a p-value of 3.3042e-27 (<0.05), indicating significant overall differences in the distribution of turns across different interaction patterns. This indicates that at least one pattern differs markedly from the others in terms of median turns. Subsequently, pairwise comparisons via Dunn's post-hoc test (with Bonferroni p-value correction) pinpoint the specific sources of these differences. As shown in Table XX, the p-value between the linear and tree patterns stands at 4.1771e-27 (<0.05), and that between the star and tree patterns at 3.5661e-15 (<0.05), while no significant difference emerges between the linear and star patterns. These results imply that the turn distributions for linear and star patterns exhibit high similarity, whereas the tree pattern distinctly diverges from both, typically associating with longer interaction turns.


%The four students divide into two groups, with two graduate students per group. Each annotator assesses the card content based on their understanding and assigns the appropriate task type.
%We collect the annotation results from both student groups and perform initial statistical analysis. 
%For classification conflicts that arise during annotation, we retain the disputed cards and organize group discussions among team members, facilitating extensive exchanges and arguments until achieving agreement.
%If new task types emerge during annotation, the student team consults with the expert analysis team for in-depth discussion and confirmation of inclusion. 
%To further evaluate inter-annotator consistency, we calculate Cohen's Kappa for each team, resulting in an average value of 0.85, which demonstrates high reliability and stability in the annotation outcomes. 
%Through this systematic analysis, we obtain a total of 5 task types (encompassing 12 subtypes) and 11 instruction intents. As shown in Table xx.


%% =========图定义============
% Subsequently, we modeled the human-LLM interaction process using graph theory to describe interaction patterns formally.
% %% 交互模式的形式化定义  --- todo
% \bin{formanlly pattern}

% \textbf{Basic Graph Model Definition}
% Let $G = (V, E)$ denote a directed acyclic graph that represents a complete interaction dialogue, where $V$ is the set of nodes, and each node $v\in V$ corresponds to an interaction turn, formalized as an ordered pair $v= (q_{u},r_{i})$.
% Here, $q_{u}$ is the user's query text, and $r_{i}$ is the LLM's response text. Each node $v$ encapsulates the minimal unit of interaction, ensuring independence and traceability for every turn. 
% The total number of nodes $\left | V \right |$ indicates the dialogue length.

% The set $ E \subseteq V \times V $ comprises directed edges, where an edge $ (u, v) \in E  $ signifies that turn $v$ directly follows turn $u$, meaning the user query in $v$ semantically depends on the LLM response in $u$.

% We introduce a virtual root node $v_0 \notin V$  (containing no actual interaction content) and add edges $(v_0, v_r) $ to all actual root nodes $v_r$ (nodes with in-degree 0), thereby extending the graph to \( G' = (V \cup \{v_0\}, E \cup \{(v_0, v_r) \mid \deg^-(v_r) = 0\}) \). This ensures a single root node. 
% Termination nodes (with out-degree 0) represent the absence of further interaction.
% Based on this graph model, we formalize three primary interaction patterns, each defined through the topological structure of the graph, which remains a directed acyclic graph.


% \textbf{Linear Pattern}
% The extended graph \( G' \) forms a directed path, featuring a unique sequence of nodes \( v_0, v_1, v_2, \dots, v_n \) (where \( n = |V| \geq 0 \)), such that \( E' = \{(v_i, v_{i+1}) \mid 0 \leq i < n\} \). In this structure, the root node \( v_0 \) has in-degree 0 and out-degree 1 (if \( n > 1 \)); the termination node \( v_n \) has in-degree 1 (if \( n > 1 \)) and out-degree 0; and all intermediate nodes \( v_i \) (for \( 0 < i < n \)) have in-degree and out-degree both equal to 1. The graph contains no cycles or branches, with a unique path of length \( n \) and diameter \( n \).


% \textbf{Star Pattern}
% The extended graph \( G' \) forms a directed star, featuring a unique central node \( v_0 \), such that \( E' = \{(v_0, v_i) \mid v_i \in V\} \). In this structure, the central node \( v_0 \) has in-degree 0 and out-degree \( |V| \); all leaf nodes \( v_i \) have in-degree 1 and out-degree 0. The graph contains no cycles or crossing edges, with depth 1 (all paths have length at most 1) and diameter 1.


% \textbf{Tree Pattern}
% The extended graph \( G' \) forms a directed tree, constituting a connected acyclic directed graph with a unique root node \( v_0 \) (in-degree 0), where the path from \( v_0 \) to any other node is unique. In this structure, the root node \( v_0 \) has in-degree 0 and out-degree at least 0; all non-root nodes have in-degree exactly 1 and out-degree at least 0 (permitting branches).

%% =========图定义============

% The Kruskal-Wallis H test serves as a non-parametric statistical method for comparing the medians of three or more independent sample groups to determine if significant differences exist. 
% It acts as a non-parametric alternative to one-way analysis of variance (ANOVA), proving particularly useful when data fail to meet assumptions of normality or homogeneity of variance. 
% Specifically, this test ranks all samples and computes the rank sum statistic H to assess inter-group differences. 
% The H value approximates a chi-square distribution, allowing computation of a p-value to decide whether to reject the null hypothesis (that all group medians are equal).


% Dunn's post-hoc test constitutes a multiple comparison procedure applied after the Kruskal-Wallis H test identifies significant inter-group differences. It facilitates pairwise comparisons to pinpoint which specific group pairs exhibit statistically significant differences. 
% This test relies on standardized rank differences and incorporates Bonferroni correction or other adjustments to control the false positive rate in multiple comparisons, thereby ensuring the accuracy and reliability of the results.

% \bin{Are these introductions able to be shorter?}



% We examined the relationship between interaction turns and interaction patterns using a Kruskal-Wallis H test. The test reveals a significant overall difference in the distribution of turns across patterns (p < 0.05), indicating that the median turn count of at least one pattern differed from the others.
% To identify specific differences, we conducted Dunn's post-hoc test with Bonferroni correction. The results, shown in Table XX, indicates that the tree pattern had significantly more interaction turns than both the linear (p < 0.05) and star (p < 0.05) patterns. In contrast, no significant difference was found between the linear and star patterns.
% These findings suggest that while linear and star patterns have similar turn counts, the tree pattern is associated with distinctly longer interactions.



% =========任务类型与交互模式分析============

% We then analyzed standardized residuals to pinpoint specific relationships (see Table ~\ref{rq_1_std}), where absolute values >1.96 indicate significance and >1.0 suggest a tendency. 
%Second, query information tasks yield a residual of 2.520 with the star pattern (absolute value > 1.96), revealing a significant preference for the star pattern. These tasks frequently entail retrieving information or addressing queries from diverse perspectives, where the star pattern supports divergent interactions centered on a core theme, such as branching from one knowledge point to interconnected ones. This underscores users' propensity for exploratory exchanges in knowledge-dense contexts.




% As illustrated in Figure XX, these shifts appear in the density distributions of turns in patterns and task types. Linear modes concentrate at lower turns for most tasks. In contrast, tree modes extend toward higher turns. They exhibit broader variability in tasks such as design-driven development and environment configuration.






==> copy/5_following.tex <==
\section{RQ2: LLM Instruction Following Capabilities}

\subsection{Methodology}
%To assess the instruction-following capability of LLMs during human-LLM interactions, we employ a dual evaluation mechanism that examines LLM responses across multi-turn conversations. 
\bin{To evaluate the instruction-following ability of LLMs in human-LLM interactions, we adopted a dual evaluation mechanism that assesses LLM responses in multi-turn conversations.}

Specifically, we first selected DeepSeek-reasoner \cite{} as the primary evaluator, which has acquired advanced reasoning abilities through reinforcement learning, including features such as self-verification and reflection. It excels in complex instruction evaluation tasks and handles multi-layered instruction analysis effectively. We provided DeepSeek-reasoner with custom prompts, as shown in Figure XX. These prompts include the full dialogue context, user instructions, and LLM responses, which require the model to analyze turn by turn whether each response fully adheres to the instructions. %To optimize evaluator performance, we use default parameter settings.
\bin{Default parameter settings were employed to optimize evaluator performance.}

Second, to ensure result reliability, we conducted manual sampling validation on DeepSeek outputs. The sampling covers 20\% of the data and spans all five task types. Validators consist of two experts from the expert team and two graduate students from the annotation team. All possess extensive experience in LLM interaction analysis. The validation process follows an independent assessment protocol. Each validator reviewed samples individually and assigned instruction-following classifications. For samples with discrepancies, we resolved them via majority voting to minimize subjective bias. Ultimately, manual validation results align with DeepSeek outputs at over 85\% consistency. This confirms the automated evaluator's effectiveness and bolsters the credibility of our experimental conclusions.

Finally, drawing from the MultiIF framework[update], this study introduces three key metrics to quantify LLM instruction-following and forgetting abilities. 
\bin{forgetting ability? Sounds inappropriate}

Instruction-level Strict Accuracy (ISA) : measures the proportion of instances where the model accurately follows individual instructions. This metric focuses on whether the model completes each isolated instruction task without error. It emphasizes precision in single-instruction execution.

[ISA Equation]

Conversation-level Strict Accuracy (CSA):  evaluates the model's accuracy across an entire multi-turn dialogue. It assesses whether the model correctly executes every user instruction from the dialogue start up to the current turn. This metric highlights the model's capacity for sustained understanding and execution in multi-turn interactions.

[CSA Equation]

Instruction Forgetting Ratio (IFR) : quantifies the proportion of previously correctly followed instructions that the model forgets in subsequent turns of a multi-turn dialogue. It specifically captures cases where the model fails to adhere to an instruction that it executed correctly in an earlier turn.

[IFR Equation]


[prompt template]


\subsection{Result and analysis}
We observed that the instruction-level strict accuracy in multi-turn conversation data is 48.24\%, while the conversation-level strict accuracy is only 24.07\%. Figure XX shows that, in multi-turn conversations, different LLMs exhibit relatively high non-compliance rates, ranging from approximately 20\% in standout models like MPT-30b-Chat to about 80\% in models such as RWKV-4-Raven. This indicates a common challenge in maintaining instruction adherence during prolonged conversations.

% 条形图 
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq2_tiao.pdf}
    \caption{Distribution of Instruction Compliance and Non-Compliance Across Different LLMs} 
    \label{ImplicitRequirement}
    \vspace{-0.4cm}
\end{figure}


\subsubsection{conversation-level}
The conversation-level strict accuracy (i.e., the proportion of conversations in which all instructions are followed correctly) stands at only 24.07\%. This finding indicates that, in the entire dataset, the majority of conversations (approximately 75.93\%) involve at least one instance of instruction non-compliance. To further explore the underlying reasons for the weak instruction-following capabilities of LLMs, we conducted an analysis from the perspectives of task types and interaction modes.


% 任务与指令不遵循
\textbf{Tasks and Instruction Non-Compliance}
We hypothesize that different task types lead to significant differences in LLMs' instruction-following capabilities. 
Given the non-normal distribution of instruction non-compliance data, we employed the Kruskal-Wallis H test to compare median differences in non-compliance rates across task types and thus test this hypothesis. Results yield a p-value of 0.6658(>0.05). 


%This outcome shows that we cannot reject the null hypothesis, indicating no statistically significant impact of task types on LLM failure to follow instructions. While LLMs exhibit no significant differences in non-compliance across high-level task categories, this does not preclude systematic variations at the finer-grained subtask level.
\bin{Despite the lack of statistically significant differences across high-level task categories, systematic variations may still exist at the subtask level.} 
Accordingly, we conducted a more detailed analysis to examine how specific subtask types influence non-compliance. In this step, we continued to employ the Kruskal-Wallis H test to compare, in a non-parametric manner, median differences in instruction non-compliance data across different subtask types. 
Experimental results indicate that the p-value of 0.04 (< 0.05) reflects a statistically significant impact of subtask types on failure to follow instructions in LLMs.
%This significance indicates that LLM performance varies not uniformly across high-level categories but rather depends on the characteristics of specific subtasks.
\bin{The significance implies that variation in LLM performance is driven primarily by subtask-specific factors rather than general task categories.}


A closer examination of adherence rate distributions across subtasks, as illustrated in Figure XX, reveals substantial variability in non-compliance rates. Notably, the database knowledge query subtask shows the lowest non- compliance rate (38.46\%), which indicates LLM's strong instruction compliance in handling structured queries. This likely stems from the deterministic nature of such tasks and the standardized aspects of knowledge retrieval. In contrast, code generation, code refactoring, tool development, and environment configuration and deployment exhibit the highest non-compliance rates, at 87.50\%, 86.96\%, 82.05\%, and 81.82\%, respectively. These tasks typically involve intricate generation or modification processes, which heighten the risk of instruction non-compliance. 


Other subtasks, including code explanation (74.58\%), data science and machine learning (71.43\%), bug fixing (70.15\%), and functional expansion (70.73\%), display intermediate non-compliance rates, reflecting moderate challenges. For instance, bug fixing often requires iterative repairs, while data science and machine learning tasks entail modifications to complex models. These differences underscore that, in coding-related interactions, generation and modification subtasks more readily provoke instruction non-compliance than query-based subtasks. Such insights guide future efforts to enhance LLMs' multi-turn instruction-following capabilities.


% 子任务条形图
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq2_sub_task.pdf}
    \caption{Distribution of Instruction Following and Non-Compliance Across Different Subtask Types} 
    \label{ImplicitRequirement}
    \vspace{-0.4cm}
\end{figure}



% finding 4
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 4:}
Code generation, code refactoring, tool development, and environment configuration and deployment commonly provoke non-compliance, with rates exceeding 80\%. Code explanation, data science and machine learning, bug fixing, and functional expansion show comparable challenges, exhibiting rates of failure to follow instructions of approximately 70\% to 75\%.

\end{tcolorbox}

\textbf{Interaction Patterns and Instruction Non-Compliance}

%We hypothesize that different interaction modes, such as linear, star, and tree, may lead to significant variations in LLM instruction non-compliance rates. To test this, we employed the Kruskal-Wallis H test. Results yield a p-value of 1.265e-04(<0.05). This confirms substantial overall differences in median non-compliance rates across these modes. Such findings indicate that interaction modes exert a non-random influence on LLMs' overall instruction adherence.
\bin{We hypothesize that interaction modes (linear, star, tree) influence LLMs’ instruction compliance rate. A Kruskal-Wallis H test confirms this, revealing a significant difference in median non-compliance rates (p = 1.265e-04). These results suggest that interaction structure non-randomly influences LLM's instruction adherence.}

To further examine average non-compliance rates, we computed statistics on instruction non-following under each mode. As shown in Table xxx, the tree pattern exhibits the highest rate (94.29\%), showing that LLMs in tree interactions almost invariably omit or deviate from at least one instruction. The linear pattern follows at 73.49\%, while the star mode shows the lowest rate (64.41\%). This distribution implies that the star pattern, despite its multi-branching nature, benefits from a structure centered on a core topic, which may ease LLMs' context management. In contrast, the deep branching in the tree pattern markedly amplifies challenges.


\bin{[Interaction Mode Statistics tab]}
% finding 5
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 5:}
The tree pattern emerges as a "high-risk" pattern for failures to follow instructions. 
Its non-compliance rate significantly exceeds that of the other two (p < 0.05). In contrast, the linear and star patterns show no significant differences.


\end{tcolorbox}

% 指令级别
\subsubsection{instruction-level}
\textbf{Turns and Instruction Non-Compliance}
To uncover the spatiotemporal distribution patterns of instruction non-compliance in LLM-human interactions, we investigated the positional preferences for such occurrences, specifically whether they tend to emerge in the early or late stages of conversations.
%We first categorize conversations into short (turn $\leq$4) and long (turn>4) based on prior analyses of interaction patterns and turn counts, where turn=4 mark a pivotal transition point. Short conversations predominantly follow linear patterns, whereas long conversations often evolve into tree-like structures with markedly increased complexity. 
\bin{We've already introduced this in the last section}
For short conversations 
\bin{(turn$\leq$4)}, given their limited and fixed number of turns, we employed absolute position statistics (positions 1 through 4) to precisely capture early deviations. For long conversations \bin{(turn>4)}, which exhibit substantial variability in turn counts (ranging from 5 to dozens), we adopted a relative position binning strategy. This approach normalizes dialogue length into five equal-width intervals: Early (1-20\%), Early-Mid (21-40\%), Mid (41-60\%), Mid-Late (61-80\%), and Late (81-100\%), thereby mitigating the influence of absolute turn differences. 
%Then, we apply the Kolmogorov-Smirnov (KS) test to assess whether the distribution of non-compliance positions deviates from uniformity. If p < 0.05, we reject the uniformity hypothesis, which indicates the presence of significant bias.
\bin{We then applied the Kolmogorov–Smirnov (KS) test to assess whether the distribution of non-compliance positions deviates from uniformity. A p-value below 0.05 indicates a significant deviation, suggesting positional bias.}

As shown in Table xx, short conversations exhibit a highly uneven distribution of non-compliance, concentrated primarily in the early stages: position 1 accounts for 38.68\%, position 2 peaks at 41.22\%, position 3 drops to 14.25\%, and position 4 stands at only 5.85\%. The KS test yields 1.4088e-31 (far below 0.05), confirming significant non-uniformity. In long conversations, the distribution is comparatively flatter yet clearly skewed toward later stages: the Early interval comprises 16 Fang, 48\%, Early-Mid 18.35\%, Mid 17.98\%, Mid-Late 19.85\%, and Late reaching the highest at 27.34\%. The KS test produces a p-value of 5.798e-06 (p < 0.05), likewise endorsing non-uniform distribution, with the latter 40\% cumulatively representing 47.19\%, underscoring late-stage clustering.

%% 这个图不放了
% As depicted in Figure xxx, non-compliance in short conversations cluster heavily in the initial phases, potentially arising from LLMs' misinterpretation of starting instructions or failures in rapid context building. In contrast, long conversations manifest more non-compliance in the later phases, attributable possibly to factors like attention decay from extended sequence lengths, accumulated errors, or context overload, which may compound losses in debugging efficiency.


\bin{[tab + fig]}

% finding 6
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 6:}
In short conversations, instruction non-compliance commonly occurs at turn 2. In long dialogues, instruction non-compliance tends to occur in the late portion (i.e., 81-100\% of total turns), which corresponds to the last 20\%.

\end{tcolorbox}

\textbf{Instruction Intent and Instruction Non-Compliance }

To investigate the impact of instruction intent types on LLMs' ability to follow instructions, we hypothesize that different intent types lead to significant variations in failure rates. We first applied a chi-square test, which yields a p-value of 1.487918e-18(<0.05). This result indicates that LLMs' compliance performance depends on instruction intents rather than occurring independently, as it reflects systematic influences from their inherent characteristics.


We further examined the distribution of failure rates across instruction intent types, as shown in Table XX. Intent types such as questioning LLM responses, refactoring code, fixing bugs, and requesting code implementation exhibit high failure rates, exceeding 70\%, 60\%, 60\%, and 50\%, respectively. These intents typically involve code modifications, error corrections, or new functionality implementations, which require LLMs to handle complex constraints and contexts. In contrast, intents such as querying information and clarifying requirements show lower failure rates, approaching 45\% and 50\%. This pattern highlights the relative simplicity and determinism of query-based tasks, which facilitate accurate responses from LLMs. Intents such as adding new features and reviewing code fall in between, indicating moderate levels of challenge.

The expected frequency analysis in Figure XX further uncovers deviation trends. For intents like fixing bugs and refactoring code, observed failure rates surpass expectations, whereas query-based intents, such as querying information, display observed instruction following rates above expectations. This suggests that LLMs deviate more readily when handling intents that demand corrective or iterative processes.


The standardized residuals in Table XX further delineate these differences. For the fix bugs intent, the residual for compliance registers at -2.08, while that for non-compliance reaches 2.00, indicating a significant bias toward failure. The question LLM response intent yields residuals of -1.75 and 1.68, approaching the significance threshold and suggesting a tendency toward non-compliance. In contrast, the query information intent produces residuals of 1.65 and -1.59, revealing a clear positive orientation toward compliance. Meanwhile, the refactor code and request code implementation intents exhibit absolute residual values exceeding 1.0, underscoring noteworthy negative deviations.



\bin{[tab + fig]}

% 期望图
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq2_qiwang.pdf}
    \caption{Instruction Non-Compliance Rates Across Instruction Types with 95\% Confidence Intervals} 
    \label{ImplicitRequirement}
    \vspace{-0.4cm}
\end{figure}


% finding 7
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 7:}
Intents such as fixing bugs, refactoring code, and questioning LLM responses exhibit high rates of non-compliance and prove prone to errors. In contrast, querying information demonstrates significantly better following of instructions.

\end{tcolorbox}


% 指令遗忘
\subsubsection{Instructions Forgetting}

We also observed instruction forgetting in LLMs. %Here, we define the forgetting step length as the interval between the turn where an instruction intent type first appears and the turn where failure to follow instructions first occurs.
\bin{Here, the forgetting step length is defined as the interval between the first appearance turn and the first failure turn of a certain instruction intent type.}
If an intent type never results in failure to follow instructions, we exclude it from forgetting events. First, based on DeepSeek's detection results, we tracked each instruction intent's initial appearance turn and first failure turn across individual conversations. We then re-examined these cases to confirm forgetting and compute the intervals as forgetting step lengths. Next, we aggregated the distribution of step lengths across all forgetting events to quantify the temporal characteristics of forgetting.

As shown in Table XX, the forgetting step length distribution exhibits a right-skewed long-tail shape, with a total of 46 forgetting events. Step lengths of 1 and 2 account for the highest proportions, at approximately 26\% and 33\%, respectively, together exceeding 58\%. Step lengths from 3 to 8 decrease progressively, while those exceeding 5 represent only about 4\%. Cumulative proportions further indicate that roughly 59\% of forgetting occurs within step lengths of 2, and about 87\% within 4. The mean step length stands at approximately 2.65 turns, showing that forgetting typically emerges within around 3 turns. 

% 指令遗忘表格
\bin{[tab + fig]}

% finding 8
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 8:}
We observed that during interactions, approximately 80\% of instructions undergo forgetting within 4 turns, with an average forgetting step length of 3.

\end{tcolorbox}





==> copy/5_following_1.tex <==
\section{RQ2: LLM Instruction Following Capabilities}

\subsection{Methodology}

To evaluate the instruction-following ability of LLMs in human-LLM interactions, we adopted a dual evaluation mechanism that assesses LLM responses in multi-turn conversations.
Given the large scale and diversity of interactions in the WildChat and LMSYS-Chat-1M datasets, we employ LLM-based automatic evaluation rather than predefined test cases to enhance scalability.
Specifically, we first selected DeepSeek-reasoner \cite{} as the primary evaluator, which has acquired advanced reasoning abilities through reinforcement learning, including features such as self-verification and reflection. It excels in complex instruction evaluation tasks and handles multi-layered instruction analysis effectively. 
We provide DeepSeek-Reasoner with custom prompts (details in the data link), incorporating full dialogue context, user instructions, and LLM responses, to evaluate turn-by-turn if each response fully complies with the instructions.
Default parameter settings were employed to optimize evaluator performance.

Second, to ensure result reliability, we conducted manual sampling validation on DeepSeek outputs. The sampling covers 20\% of the data and spans all five task types. Validators consist of two experts from the expert team and two graduate students from the annotation team. All possess extensive experience in LLM interaction analysis. The validation process follows an independent assessment protocol. Each validator reviewed samples individually and assigned instruction-following classifications. For samples with discrepancies, we resolved them via majority voting to minimize subjective bias. Ultimately, manual validation results align with DeepSeek outputs at over 85\% consistency. This confirms the automated evaluator's effectiveness and bolsters the credibility of our experimental conclusions.


Finally, we introduce instruction-level loose accuracy and conversation-level loose accuracy in MultiIF~\citet{he2024multi} to quantify the instruction-level and conversation-level following capabilities of the LLMs.
Instruction-level loose accuracy measures the consistency of individual LLM responses to user instructions under a relaxed criterion. 
It handles introductory phrases, such as ``Certainly, here is the revised version ''.
Conversation-level loose accuracy assesses overall dialogue compliance between users and LLMs using the same relaxed standard.




\subsection{Result and analysis}
\song{Which table/figure do you show the performance?}
% % ==========总体情况=============
% We observed that the instruction-level loose accuracy in multi-turn conversation data is 48.24\%, while the conversation-level loose accuracy is only 24.07\%. Figure XX shows that, in multi-turn conversations, different LLMs exhibit relatively high non-compliance rates, ranging from approximately 20\% in standout models like MPT-30b-Chat to about 80\% in models such as RWKV-4-Raven. This indicates a common challenge in maintaining instruction adherence during prolonged conversations.

% % 条形图 
% \begin{figure}%[H]
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     \includegraphics[width=0.45\textwidth]{fig/rq2_tiao.pdf}
%     \caption{Distribution of Instruction Compliance and Non-Compliance Across Different LLMs} 
%     \label{ImplicitRequirement}
%     \vspace{-0.4cm}
% \end{figure}
% % ==========总体情况=============

\subsubsection{Conversation-level following capability}
The conversation-level loose accuracy (i.e., the proportion of conversations in which all instructions are followed correctly) stands at only 24.07\%. This finding indicates that, in the entire dataset, the majority of conversations (approximately 75.93\%) involve at least one instance of instruction non-compliance. To further explore the underlying reasons for the weak instruction-following capabilities of LLMs, we conducted an analysis from the perspectives of task types and interaction modes.

\song{unclear how these two types of non-compliance were summarized, currently you said "hypothesize", this could be a problem; often these claims should be made based on observations of your data or results}
% 任务与指令不遵循

\textbf{Tasks and Instruction Non-Compliance}
We hypothesize\song{any reference} that different task types lead to significant differences in LLMs' instruction-following capabilities. 
Since the instruction non-compliance data are non-normal distributed, we employ Kruskal-Wallis H to test the hypothesis.
Results yield a p-value of 0.6658(>0.05). 
Despite the lack of statistically significant differences across high-level task categories, systematic variations may still exist at the subtask level.
Accordingly, we conducted a more detailed analysis to examine how specific subtask types influence non-compliance. In this step, we continued to employ the Kruskal-Wallis H test to compare, in a non-parametric manner, median differences in instruction non-compliance data across different subtask types. 
Experimental results indicate that the p-value of 0.04 (< 0.05) reflects a statistically significant impact of subtask types on failure to follow instructions in LLMs.
The significance implies that variation in LLM performance is driven primarily by subtask-specific factors rather than general task categories.


A closer examination of adherence rate distributions across subtasks, as illustrated in Figure ~\ref{subtask_non}, reveals substantial variability in non-compliance rates. 
Notably, the database knowledge query subtask shows the lowest non-compliance rate (38.46\%), which indicates LLM's strong instruction compliance in handling structured queries. This likely stems from the deterministic nature of such tasks and the standardized aspects of knowledge retrieval. In contrast, code generation, code refactoring, tool development, and environment configuration and deployment exhibit the highest non-compliance rates, at 87.50\%, 86.96\%, 82.05\%, and 81.82\%, respectively. These tasks typically involve intricate generation or modification processes, which heighten the risk of instruction non-compliance. 


Other subtasks, including code explanation (74.58\%), data science and machine learning (71.43\%), bug fixing (70.15\%), and functional expansion (70.73\%), display intermediate non-compliance rates, reflecting moderate challenges. For instance, bug fixing often requires iterative repairs, while data science and machine learning tasks entail modifications to complex models. These differences underscore that, in coding-related interactions, generation and modification subtasks more readily provoke instruction non-compliance than query-based subtasks. Such insights guide future efforts to enhance LLMs' multi-turn instruction-following capabilities.


% 子任务条形图
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq2_sub_task.pdf}
    \caption{Distribution of Instruction Following and Non-Compliance Across Different Subtask Types} 
    \label{subtask_non}
    \vspace{-0.4cm}
\end{figure}



% finding 4
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 4:}
Code generation, code refactoring, tool development, and environment configuration and deployment commonly provoke non-compliance, with rates exceeding 80\%. Code explanation, data science and machine learning, bug fixing, and functional expansion show comparable challenges, exhibiting rates of failure to follow instructions of approximately 70\% to 75\%.

\end{tcolorbox}


\textbf{Interaction Patterns and Instruction Non-Compliance}

We hypothesize that interaction modes influence LLMs’ instruction compliance rate. 
A Kruskal-Wallis H test confirms this, revealing a significant difference in median non-compliance rates (p = 1.265e-04). These results suggest that interaction structure non-randomly influences LLM's instruction adherence.

To further examine average non-compliance rates, we computed statistics on instruction non-compliance under each mode. As shown in Table ~\ref{rq_2_std}, the tree pattern exhibits the highest rate (94.29\%), showing that LLMs in tree interactions almost invariably omit or deviate from at least one instruction. The linear pattern follows at 73.49\%, while the star mode shows the lowest rate (64.41\%). This distribution implies that the star pattern, despite its multi-branching nature, benefits from a structure centered on a core topic, which may ease LLMs' context management. In contrast, the deep branching in the tree pattern markedly amplifies challenges.



\input{tab/rq_2_std}

% finding 5
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 5:}
The tree pattern emerges as a "high-risk" pattern for failures to follow instructions. 
Its non-compliance rate significantly exceeds that of the other two (p < 0.05). In contrast, the linear and star patterns show no significant differences.


\end{tcolorbox}


% 指令级别
\subsubsection{Instruction-level following capability}
\song{this part directly starts from the non-compliance; may need to discuss the performance first, then the reasons for noncompliance}

\bin{need merge }
\textbf{Turns and Instruction Non-Compliance}
To uncover the spatiotemporal distribution patterns of instruction non-compliance in LLM-human interactions, we investigated the positional preferences for such occurrences, specifically whether they tend to emerge in the early or late stages of conversations.


For short conversations (turn$\leq$4), given their limited and fixed number of turns, we employed absolute position statistics (positions 1 through 4) to precisely capture early deviations. For long conversations (turn>4), which exhibit substantial variability in turn counts (ranging from 5 to dozens), we adopted a relative position binning strategy. This approach normalizes dialogue length into five equal-width intervals: Early (1-20\%), Early-Mid (21-40\%), Mid (41-60\%), Mid-Late (61-80\%), and Late (81-100\%), thereby mitigating the influence of absolute turn differences. 
We then applied the Kolmogorov–Smirnov (KS) test to assess whether the distribution of non-compliance positions deviates from uniformity. A p-value below 0.05 indicates a significant deviation, suggesting positional bias.

As shown in Table ~\ref{rq_2_turn}, short conversations exhibit a highly uneven distribution of non-compliance, concentrated primarily in the early stages: position 1 accounts for 38.68\%, position 2 peaks at 41.22\%, position 3 drops to 14.25\%, and position 4 stands at only 5.85\%. The KS test yields 1.4088e-31 (far below 0.05), confirming significant non-uniformity. In long conversations, the distribution is comparatively flatter yet clearly skewed toward later stages: the Early interval comprises 16 Fang, 48\%, Early-Mid 18.35\%, Mid 17.98\%, Mid-Late 19.85\%, and Late reaching the highest at 27.34\%. The KS test produces a p-value of 5.798e-06 (p < 0.05), likewise endorsing non-uniform distribution, with the latter 40\% cumulatively representing 47.19\%, underscoring late-stage clustering.

% 指令不遵循的 位置分布
\input{tab/rq_2_turn}

% finding 6
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 6:}
In short conversations, instruction non-compliance commonly occurs at turn 2. In long dialogues, instruction non-compliance tends to occur in the late portion (i.e., 81-100\% of total turns), which corresponds to the last 20\%.

\end{tcolorbox}

\textbf{Instruction Intent and Instruction Non-Compliance }

To investigate the impact of instruction intent types on LLMs' ability to follow instructions, we hypothesize that different intent types lead to significant variations in failure rates. We first applied a chi-square test, which yields a p-value of 1.4879e-18(<0.05). This result indicates that LLMs' compliance performance depends on instruction intents rather than occurring independently, as it reflects systematic influences from their inherent characteristics.


We further examined the distribution of failure rates across instruction intent types, as shown in Table ~\ref{rq_2_intent}. Intent types such as questioning LLM responses, refactoring code, fixing bugs, and requesting code implementation exhibit high failure rates, exceeding 70\%, 60\%, 60\%, and 50\%, respectively. 
These intents typically involve code modifications, error corrections, or new functionality implementations, which require LLMs to handle complex constraints and contexts. In contrast, intents such as querying information and clarifying requirements show lower failure rates, approaching 45\% and 50\%. This pattern highlights the relative simplicity and determinism of query-based tasks, which facilitate accurate responses from LLMs. Intents such as adding new features and reviewing code fall in between, indicating moderate levels of challenge.

Standardized residuals reveal distinct patterns in intent and compliance associations: Fix bugs intent shows significant bias toward non-compliance (residuals: -2.08 for compliance, 2.00 for non-compliance). Question LLM response intent approaches the significance threshold, trending toward non-compliance (residuals: -1.75, 1.68). Query information intent leans positively toward compliance (residuals: 1.65, -1.59), while refactor code and request code implementation intents exhibit notable negative deviations (absolute residuals >1.0).

\input{tab/rq_2_intent}

%% ==========期望频率分析 ---不放入===============
% The expected frequency analysis in Figure XX further uncovers deviation trends. For intents like fixing bugs and refactoring code, observed failure rates surpass expectations, whereas query-based intents, such as querying information, display observed instruction following rates above expectations. This suggests that LLMs deviate more readily when handling intents that demand corrective or iterative processes.
%% ==========期望频率分析 ---不放入===============

% The standardized residuals in Table ~\ref{} further delineate these differences. For fixing bugs, the residual for compliance registers at -2.08, while that for non-compliance reaches 2.00, indicating a significant bias toward failure. The question LLM response intent yields residuals of -1.75 and 1.68, approaching the significance threshold and suggesting a tendency toward non-compliance. In contrast, the query information intent produces residuals of 1.65 and -1.59, revealing a clear positive orientation toward compliance. Meanwhile, the refactored code and request code implementation intents exhibit absolute residual values exceeding 1.0, underscoring noteworthy negative deviations.


% % ==========期望图 ---- 不放了 =======
% \begin{figure}%[H]
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     \includegraphics[width=0.45\textwidth]{fig/rq2_qiwang.pdf}
%     \caption{Instruction Non-Compliance Rates Across Instruction Types with 95\% Confidence Intervals} 
%     \label{ImplicitRequirement}
%     \vspace{-0.4cm}
% \end{figure}
% % ==========期望图 ---- 不放了 =======


% finding 7
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 7:}
Intents such as fixing bugs, refactoring code, and questioning LLM responses exhibit high rates of non-compliance and are prone to errors. In contrast, querying information demonstrates significantly better following of instructions.

\end{tcolorbox}

% 指令遗忘
\subsubsection{Instructions Forgetting}
\song{this part seems unrelated to RQ2, i.e., instruction-following}

\bin{need merge}
We also observed instruction forgetting in LLMs.
Here, the forgetting step length is defined as the interval between the first appearance turn and the first failure turn of a certain instruction intent type.
If an intent type never results in failure to follow instructions, we exclude it from forgetting events. First, based on DeepSeek's detection results, we tracked each instruction intent's initial appearance turn and first failure turn across individual conversations. We then re-examined these cases to confirm forgetting and compute the intervals as forgetting step lengths. Next, we aggregated the distribution of step lengths across all forgetting events to quantify the temporal characteristics of forgetting.

As shown in Table ~\ref{rq_3_forget}, the forgetting step length distribution exhibits a right-skewed long-tail shape, with a total of 46 forgetting events. Step lengths of 1 and 2 account for the highest proportions, at approximately 26\% and 33\%, respectively, together exceeding 58\%. Step lengths from 3 to 8 decrease progressively, while those exceeding 5 represent only about 4\%. Cumulative proportions further indicate that roughly 59\% of forgetting occurs within step lengths of 2, and about 87\% within 4. The mean step length stands at approximately 2.65 turns, showing that forgetting typically emerges within around 3 turns. 

% 指令遗忘表格 
\input{tab/rq_3_forget}

% finding 8
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 8:}
We observed that during interactions, approximately 80\% of instructions undergo forgetting within 4 turns, with an average forgetting step length of 3.

\end{tcolorbox}





==> copy/6_human.tex <==
\section{RQ3: Human Satisfaction }


\subsection{Methodology}
This section employs a dual-scoring mechanism to assess human satisfaction with the interaction process.
First, we used the deepseek-reasoner to assign a five-point satisfaction score to LLM responses within conversations. 
The scoring criteria draw from the WB-Score evaluation standard in WildBench, with scores ranging from 1 (highly unsatisfactory, with severe issues) to 5 (highly satisfactory, delivering an excellent experience that exceeds expectations). 
The evaluation process adopts default parameter settings. Second, to ensure the reliability of LLM-based scoring, we conducted manual reviews following the procedure outlined in Section 5.1. 
During these reviews, we observe that users incorporate positive or negative vocabulary in their instructions to express satisfaction or dissatisfaction with LLM responses. For instance, the presence of negation words such as ``don’t'', ``no'', or ``not'' in the current instruction often indicates dissatisfaction with the previous interaction. If users highlight errors or irrelevant information in the prior LLM response during the next turn, it suggests that the LLM fails to fully implement the user's instruction correctly. Conversely, the inclusion of expressions of gratitude in the subsequent instruction signals satisfaction with the preceding LLM response. Accordingly, we integrated assessments of LLM response quality with analyses of common emotional vocabulary to evaluate human satisfaction comprehensively. The manual review results align with LLM evaluations in over 87\% of cases, establishing a solid data foundation for subsequent quantitative analysis.


\subsection{Result and analysis }

% 整体满意度分析
% \subsubsection{Overall Satisfaction Analysis}
%% 总体满意图与turn变化
% We first analyzed the relationship between satisfaction and conversation length. Since evaluating the final satisfaction for each conversation proves ineffective, we employed linear regression to examine satisfaction during the interaction process. Specifically, this involves assessing the trend in average satisfaction across all conversations at each turn. The results reveal a P-value of 0.001 (<0.05), which indicates that the negative correlation between conversation turns and satisfaction holds statistical significance. %Moreover, the slope for changes in average satisfaction stands at -0.111, implying that each additional conversation turn reduces user satisfaction by approximately 0.111 points on average. 
% \bin{I think this sentence can be deleted}

% Figure XX depicts the average satisfaction per conversation turn. As the number of turns increases, average satisfaction clearly trends downward overall.

% % 回归图
% \begin{figure}%[H]
%     \centering
%     \setlength{\abovecaptionskip}{0.1cm}
%     \includegraphics[width=0.45\textwidth]{fig/rq3_logic.pdf}
%     \caption{Linear Regression Analysis of Average User Satisfaction Trends Across Conversation Turns} 
%     \label{ImplicitRequirement}
%     \vspace{-0.4cm}
% \end{figure}


\subsubsection{Task and Human Satisfaction}

This section analyzes user satisfaction with different task types to reveal user performance and its underlying patterns.
Figure ~\ref{rq_3_pao} illustrates the average satisfaction scores for five primary task categories and their subtasks. 
Analyses reveal substantial capability variations and uneven user experiences in how models address diverse development tasks.


First, from a macro-level view of task categories, user satisfaction correlates strongly with the software development phase and the abstraction level involved. 
Tasks emphasizing conceptual design and information planning in early development stages generally elicit higher user satisfaction: design-driven developmen (average score:3.22) and information query (average score:3.18) rank highest. 
Users in these contexts often treat the LLM as a knowledgeable advisor for framework design, direction exploration, or knowledge acquisition. 
By contrast, satisfaction diminishes as tasks advance to concrete coding implementation and environment setup. Categories such as requirement-driven development (average score: 2.94), environment configuration (average score: 2.94), and code quality optimization (average score: 2.99) all register lower scores. 
Here, users expect the LLM to produce directly runnable code or configurations.
Consequently, errors, incompatibilities, or inefficiencies in outputs obstruct progress and provoke negative feedback.


Second, in-depth subtask examination provides more concrete explanations and corroboration.
Database knowledge query as the top-performing subtask, with an average score of 3.99. This pattern indicates that LLMs deliver precise, satisfying responses when users seek knowledge with well-defined structures and rules, such as database schemas or SQL syntax. In sharp contrast, Configuration debug yields the lowest average score of 2.69 across all subtasks. Such outcomes expose a fundamental LLM limitation: performance falls short in diagnostic and repair scenarios that lack standardized patterns and demand context-specific, iterative trial-and-error. Within individual major categories, subtasks further display pronounced satisfaction imbalances. 
For information query, database knowledge query (score: 3.99) substantially outperforms programming knowledge query (score: 2.93). Likewise, under environment configuration, generative subtasks like environment configuration and deployment (score: 3.16) garner significantly higher ratings than reparative ones like configuration debug (score: 2.69). These findings underscore pervasive capability asymmetries in LLMs during problem resolution.


% paopao
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq3_paopao.pdf}
    \caption{Average User Satisfaction Ratings Across Tasks and Subtasks} 
    \label{rq_3_pao}
    \vspace{-0.4cm}
\end{figure}







% finding 10
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 10:}
In human-LLM interactions, code quality optimization tasks and requirement-driven development tasks exhibit lower satisfaction levels. In contrast, structured knowledge query tasks and algorithm design tasks achieve higher satisfaction.

\end{tcolorbox}



\subsubsection{xxx}

Through an analysis of core task distributions across conversations of varying lengths, we find that user satisfaction declines as dialogues deepen. This decline stems from conversations falling into inefficient "generate-revise" cycles, which markedly increase the proportion of error-correction tasks.

As shown in Figure ~\ref{rq_3_tiao}, shorter conversations (2-4 turns) feature core tasks that center on requesting code implementation and querying information. These constructive tasks dominate at this stage. In contrast, the share of fixing bugs stays relatively low, ranging from 11.5\% to 15.1\%. However, conversations exhibit a pivotal shift starting at the 5th turn. The proportion of fixing bugs rises substantially and emerges as a key or even leading activity. For instance, this task claims the top spot in the 5th and 6th turns, with shares of 25.5\% and 27.5\%, respectively.
In longer conversations that follow, the ranking of fixing bugs varies. Yet its persistent prominence underscores the core problem. Examples include its position as the second-ranked task in the 7th turn, its return to first in the 9th turn, and its dominance at 71.4\% in dialogues reaching 14 turns. Such patterns signal that interactions devolve into prolonged error correction. Notably, certain extended turns—such as the 7th, 12th, and 13th—see tasks like querying information reclaim the lead. This pattern does not always indicate effective advancement. Instead, it often reveals users rephrasing queries or exploring alternative approaches after unsatisfactory LLM responses. Such behaviors highlight inefficiencies in the interaction.

In summary, conversation length extends in tandem with falling satisfaction, as interaction efficiency diminishes. Extended dialogues typically reflect initial LLM outputs that miss user needs. This forces additional turns for clarification, revision, or retries. The resulting move from one-shot resolutions to iterative debugging drives the satisfaction drop with increasing conversation length.


% 条形图
\begin{figure}%[H]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \includegraphics[width=0.45\textwidth]{fig/rq3_tiao.pdf}
    \caption{Distribution of Core Tasks Across Varying Conversation Lengths} 
    \label{rq_3_tiao}
    \vspace{-0.4cm}
\end{figure}


% finding 9
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 9:}
Conversations exhibit poorer performance as they lengthen, with task focus shifting toward error correction. 
\end{tcolorbox}



\subsubsection{Interaction Pattern and Human Satisfaction}

This section examines the relationships between three primary interaction patterns and user satisfaction. To capture dynamic shifts in user sentiment, analyses introduce the concept of satisfaction trajectories. Each conversation's satisfaction progression falls into distinct categories. Examples include downward trends, which denote interactions with steadily declining satisfaction; trend reversals, which represent successful shifts from low to high satisfaction; and dual-turn lows, which specifically indicate failures concluding with low satisfaction across two turns.

As Table XX illustrates, the tree pattern emerges as a primary source of poor user experiences. This pattern highlights limitations in current LLMs when handling complex, multi-path exploratory tasks. Interactions in the tree pattern extend the longest, averaging 5.7 turns per conversation. Yet this extended engagement yields diminishing returns, with final-turn average satisfaction reaching only 2.80—the lowest across all patterns. Data on satisfaction trajectory distributions in Table 3 further elucidate the underlying causes of suboptimal experiences in the tree pattern. Here, downward trends account for 17.1\% of cases, ranking highest among patterns. Such prevalence suggests that LLM performance deteriorates progressively in intricate dialogues, as models struggle to manage multiple logical threads effectively. This dynamic often culminates in user disengagement.

The star pattern, despite shorter average turns, exposes deficiencies in LLMs' ability to deliver diverse and effective alternatives. A hallmark of this pattern lies in the elevated proportion of dual-turn lows, which reaches 30.5\%. These scenarios typically arise when users express dissatisfaction with initial LLM responses and pursue varied reformulations from the same starting point to elicit better options. Repeated failures, however, prompt abrupt conversation termination.

Analyses reveal that negative experiences pervade all patterns, with LLMs proving challenging to recover from adverse cycles once initiated.
For instance, dual-turn lows dominate as the chief negative form in brief two-turn dialogues. In contrast, downward trends prevail in extended three-to-five-turn exchanges. Notably, trend reversals remain rare across patterns, underscoring the difficulty LLMs face in rebounding from early setbacks to regain user satisfaction.




\bin{[tab}

% finding 11
\begin{tcolorbox}[colback=lightgray, colframe=lightgray, boxrule=0.5pt, arc=5pt,left=5pt,right=5pt,top=5pt,bottom=5pt]
\textbf{Finding 11:}
The tree pattern emerges as a primary locus of poor user experiences, which exposes model limitations in managing complex tasks. 
Negative experience trajectories prevail across patterns, as models struggle to recover from early failures.

\end{tcolorbox}





==> copy/tab/tj.tex <==
\begin{table}[t!]
\setlength{\abovecaptionskip}{0.1cm}
\caption{Distribution of Factors Across Different LLMs}
\tiny 
\renewcommand{\arraystretch}{1.2} % 调整行高
\setlength{\tabcolsep}{3pt} % 微调列间距

\begin{tabular}{| 
    >{\centering}m{0.9cm}| % 第一列压缩宽度
    >{\centering}m{0.6cm}| % 第二列压缩间距
    >{\centering}m{1.5cm}| % 第三列加宽
    *{6}{>{\centering\arraybackslash}m{0.6cm}|}} % 数据列统一宽度
\hline
\multicolumn{3}{|>{\centering\arraybackslash}m{3.0cm}|}{\textbf{Factors}}
% \multicolumn{3}{|c|}{\textbf{Factors}} 
    & \multicolumn{3}{c|}{\textbf{CoderEval}} 
    & \multicolumn{3}{c|}{\textbf{SWE-bench}} \\
\cline{4-9}
\multicolumn{3}{|c|}{} 
    & \textbf{D-R1} & \textbf{G-2.0} & \textbf{o1} 
    & \textbf{D-R1} & \textbf{G-2.0} & \textbf{o1} \\ 
\hline

% External 部分
\multirow{4}{0.9cm}{\centering \textbf{External}} 
    & \multirow{2}{0.6cm}{\centering UID} 
    & Data Aspect 
    & \cellcolor[HTML]{E8F4E9}1.9\% 
    & \cellcolor[HTML]{BFE3CB}8.4\% 
    & \cellcolor[HTML]{D7EDE0}5.5\% 
    & \cellcolor[HTML]{E0F1E8}4.8\% 
    & \cellcolor[HTML]{D7F0E5}5.1\% 
    & \cellcolor[HTML]{EDF6F3}1.9\% \\ 
\cline{3-9} 
& & Functional Aspect 
    & \cellcolor[HTML]{6DC68B}18.5\% 
    & \cellcolor[HTML]{63BE7B}22.9\% 
    & \cellcolor[HTML]{95D2A6}20.4\% 
    & \cellcolor[HTML]{B0DFBF}14.4\% 
    & \cellcolor[HTML]{63BE7B}29.7\% 
    & \cellcolor[HTML]{9AD8A4}16.7\% \\ 
\cline{2-9} 
& \multirow{2}{0.6cm}{\centering MCI} 
    & Missing Parameter 
    & \cellcolor[HTML]{8DD4A3}12.7\% 
    & \cellcolor[HTML]{98D4A9}14.5\% 
    & \cellcolor[HTML]{CDE9D7}7.7\% 
    & \cellcolor[HTML]{E8F4EF}2.9\% 
    & \cellcolor[HTML]{EDF6F3}0.8\% 
    & \cellcolor[HTML]{E8F5E9}2.8\% \\ 
\cline{3-9} 
& & Missing Dependencies 
    & \cellcolor[HTML]{63BE7B}27.4\% 
    & \cellcolor[HTML]{63BE7B}22.9\% 
    & \cellcolor[HTML]{63BE7B}31.5\% 
    & \cellcolor[HTML]{8FCE9F}19.2\% 
    & \cellcolor[HTML]{9BD4A2}16.1\% 
    & \cellcolor[HTML]{7FC88D}21.3\% \\ 
\hline

% Internal 部分
\multirow{6}{0.9cm}{\centering \textbf{Internal}} 
    & \multirow{2}{0.6cm}{\centering UER} 
    & CoT Inconsistent 
    & \cellcolor[HTML]{8DD4A3}12.7\% 
    & \cellcolor[HTML]{A8DAB7}12.0\% 
    & \cellcolor[HTML]{B7E0C4}12.7\% 
    & \cellcolor[HTML]{A3D8B1}15.4\% 
    & \cellcolor[HTML]{A0D6A6}15.3\% 
    & \cellcolor[HTML]{A5DCAC}14.8\% \\ 
\cline{3-9} 
& & CoT Fails Key Info 
    & 0 
    & 0 
    & 0 
    & \cellcolor[HTML]{EDF6F3}1.9\% 
    & \cellcolor[HTML]{D3EFE3}5.9\% 
    & \cellcolor[HTML]{D6F0D5}5.6\% \\ 
\cline{2-9} 
& \multirow{2}{0.6cm}{\centering UIR} 
    & Boundary Handling 
    & \cellcolor[HTML]{6FC78D}17.2\% 
    & \cellcolor[HTML]{B4DFC1}10.2\% 
    & \cellcolor[HTML]{9CD5AC}18.8\% 
    & \cellcolor[HTML]{63BE7B}28.8\% 
    & \cellcolor[HTML]{8ACE94}19.5\% 
    & \cellcolor[HTML]{63BE7B}26.9\% \\ 
\cline{3-9} 
& & Missing Exception 
    & \cellcolor[HTML]{B4E3C0}8.3\% 
    & \cellcolor[HTML]{C3E5CF}7.8\% 
    & \cellcolor[HTML]{E8F4EF}1.7\% 
    & 0 
    & 0 
    & 0.9 \\ 
\cline{2-9} 
& \multirow{2}{0.6cm}{\centering QIC} 
    & Unreasonable Order 
    & 0 
    & 0 
    & \cellcolor[HTML]{EDF6F3}0.6\% 
    & \cellcolor[HTML]{D0ECDC}8.7\% 
    & \cellcolor[HTML]{C9EDDF}6.8\% 
    & \cellcolor[HTML]{CFEDCF}6.5\% \\ 
\cline{3-9} 
& & Redundant Steps 
    & \cellcolor[HTML]{EDF6F3}1.3\% 
    & \cellcolor[HTML]{EDF6F3}1.2\% 
    & \cellcolor[HTML]{EBF5F1}1.1\% 
    & \cellcolor[HTML]{E8F4EF}2.9\% 
    & \cellcolor[HTML]{EDF6F3}0.8\% 
    & \cellcolor[HTML]{E8F5E9}2.8\% \\ 
\hline
\end{tabular}
\label{tab:merged}
\vspace{-0.4cm}
\end{table}

==> tab/rq_3_forget.tex <==
\begin{table}[t!]
\setlength{\abovecaptionskip}{0.1cm}
\caption{Distribution of Forgetting Steps}
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{1.5pt}

\begin{tabular}{ 
    >{\centering\arraybackslash}m{2.0cm} 
    >{\centering\arraybackslash}m{1.0cm} 
    >{\centering\arraybackslash}m{2.0cm} }
\toprule
\textbf{Forgetting Step} & \textbf{Num} & \textbf{Proportion (\%)} \\ 
\midrule
1 & 12 & 26.09 \\ 
2 & 15 & 32.61 \\ 
3 & 6 & 13.04 \\ 
4 & 7 & 15.22 \\ 
5 & 4 & 8.70 \\ 
6 & 1 & 2.17 \\ 
8 & 1 & 2.17 \\ 
\bottomrule
\end{tabular}
\label{rq_3_forget}
\vspace{-0.4cm}
\end{table}

==> tab/rq_3_manyidu.tex <==

% \begin{table}[t]
% \centering
% \begin{tabular}{*{10}{c}}
% \toprule
% Interaction Mode & Dual-Turn Highlight & Dual-Turn Fluctuation & Dual-Turn Low & Trend Reversal & Downward Trend & Stable High & Stable Low & High Volatility & Stable/Other \\
% \midrule
% Linear & 19.3 & 21.7 & 19.3 & 6.8 & 4.4 & 4.4 & 4.4 & 0.4 & 19.3 \\
% Star & 15.3 & 8.5 & 30.5 & 5.1 & 5.1 & 11.9 & 1.7 & 0.0 & 22.0 \\
% Tree & 0.0 & 0.0 & 0.0 & 12.9 & 17.1 & 4.3 & 7.1 & 0.0 & 58.6 \\
% \bottomrule
% \end{tabular}
% \caption{xxx}
% \label{xxx}
% \end{table}



% % =====final========
\begin{table*}[t]
    \centering
    \setlength{\abovecaptionskip}{0.1cm}
    \caption{Satisfaction Trajectory Distribution by Interaction Patterns}
    \label{tab:satisfaction_trajectory_basic}

    \newcommand{\myheading}[1]{\begin{tabular}{@{}c@{}}#1\end{tabular}}

    \begin{tabular}{lccccccccc}
        \hline 
        \textbf{Patterns} & \textbf{\myheading{Dual-Turn \\ Highlight}} & \textbf{\myheading{Dual-Turn \\ Fluctuation}} & \textbf{\myheading{Dual-Turn \\ Low}} & \textbf{\myheading{Trend \\ Reversal}} & \textbf{\myheading{Downward \\ Trend}} & \textbf{\myheading{Stable \\ High}} & \textbf{\myheading{Stable \\ Low}} & \textbf{\myheading{High \\ Volatility}} & \textbf{\myheading{Stable/ \\ Other}} \\
        \hline 
        Linear & 19.3 & 21.7 & 19.3 & 6.8 & 4.4 & 4.4 & 4.4 & 0.4 & 19.3 \\
        Star   & 15.3 & 8.5  & 30.5 & 5.1 & 5.1 & 11.9& 1.7 & 0.0 & 22.0 \\
        Tree   & 0.0  & 0.0  & 0.0  & 12.9& 17.1& 4.3 & 7.1 & 0.0 & 58.6 \\
        \hline 
    \end{tabular}
    \label{rq_3_manyidu}
    \vspace{-0.4cm}
\end{table*}



